Shuffle Private Stochastic Convex Optimization

In shuffle privacy, each user sends a collection of randomized messages to a trusted shuffler, the shuffler randomly permutes these messages, and the resulting shuffled collection of messages must satisfy differential privacy. Prior work in this model has largely focused on protocols that use a single round of communication to compute algorithmic primitives like means, histograms, and counts. We present interactive shuffle protocols for stochastic convex optimization. Our protocols rely on a new noninteractive protocol for summing vectors of bounded $\ell_2$ norm. By combining this sum subroutine with mini-batch stochastic gradient descent, accelerated gradient descent, and Nesterov's smoothing method, we obtain loss guarantees for a variety of convex loss functions that significantly improve on those of the local model and sometimes match those of the central model.

==> app_text/app-protocol.tex <==


\section{Analysis of protocol}
\label{sec:app-protocol}

\begin{lemma}
\label{lem:sum-bbgn}
The BBGN protocol~\cite{BBGN19} is $\nu_1$-biased, $\nu_2$ bounded and $\nu_3$-approximately scale invariant with $\nu_1 = 1/\poly(n, d)$, $\nu_2 = \frac{1}{\eps}$ and $\nu_3 = O(1)$.
\end{lemma}
\begin{proof}
We first sketch the BBGN protocol. 
For ease of notation, we assume the the $i$-th user receives a real number $x_i \in [0,1]$ and the goal is to compute $\sum_{i\in [n]}x_i$ under the the constraints of privacy.
For each number $x_i$, the user first rounds it to an integer $\mathsf{fp}(x_i,p) = \lfloor x_i p \rfloor + \text{Ber}(x_i p - \lfloor x_i p \rfloor)$, here $\text{Ber}(\mu)$ denotes a Bernoulli variable with mean $\mu$ (see Step 1 below).
Conceptually, the next step is to add a (discrete) Laplace noise to the summation $\sum_{i\in [n]}\mathsf{fp}(x_i, p)$. Since a discrete Laplace variable can be decomposed as the summation of $n$ difference Polya variables, each individual user can add the Polya variables to $\mathsf{fp}(x_i,p)$ and simulate the discrete Laplace distribution (see Step 2).
\footnote{Technically, let $X_i$ and $Y_i$ are independent $\mathsf{Polya}(1/n, \alpha)$ random variables, then $Z= \sum_{i=1}^{n}X_i - Y_i$ follows a discrete Laplace distribution with $\Pr[Z = k]\propto \alpha^{|k|}$.}
Finally, the user follows a $\sigma$-secure summation protocol over a finite field $\mathbb{Z}_{q}$ (which is build upon the shuffle protocol), and submit the messages to the shuffler. 
The $\sigma$-secure summation protocol guarantees to return the summation, and for any $(y_1, \cdots, y_n), (z_1, \cdots, z_n) \in \mathbb{Z}_{q}^{n}$, if $\sum_{i\in [n]}y_i = \sum_{i \in [n]}z_i (\mathsf{mod} \, q)$, then the TV distance between the protocol is less than $2^{-\sigma}$. 
Together with the Laplace (or Polya) variable we add, one can conclude the privacy of the protocol.
Concretely, for each user, its local randomize protocol works as follow.
\begin{enumerate}
    \item Round $x_i$ to $fp(x_i,p) = \lfloor x_i p \rfloor + \text{Ber}(x_i p - \lfloor x_i p \rfloor)$.
    \item Add noise $\eta \sim \mathsf{Polya}(1/n, e^{-\eps/p}) - \mathsf{Polya}(1/n, e^{-\eps/p})$. 
    \item Follow the $\sigma$-secure summation protocol and submit messages.
\end{enumerate}

The central protocol aggregate the messages and computes the summation $s$. It returns $s/p$ if $s \leq \frac{np + q}{2}$; and it returns $(s-q)/p$ otherwise. The later step is to address the potential underflow of the sum in $\mathbb{Z}_{q}$. We take a different set of parameters from the original paper (Lemma 4.1~\cite{BBGN19}) and set $p = nd$, $q = 4n^2d^2$, this will only blow up the message size by a constant factor.

In general, our protocol simulates the discrete Laplace noise, hence we expect it satisfies all properties a discrete Laplace distribution has. 
The only exception happens in the case that the total noise added has magnitude greater than $q/2$, and we call it a bad event. The bad event could cause unexpected rounding in a finite field and but it happens with probability at most $O(e^{-\eps nd})$. 
The rounding part is unbiased, the discrete Laplace noise is unbiased, and the result can be biased only when the bad event happens, i.e. the total noise is greater than $q/2$. Hence, the expected bias is within $O(q)\cdot O(e^{-\eps nd}) \leq 1/\poly(n, d)$, i.e. $\nu_1 = 1/\poly(n, d)$. 
The variance comes from three parts, the first is from the rounding part, which is at most $n/4p^2 \leq 1/4d$, the second comes from the discrete Laplace noise, and it can be at most $\eps^2$, the last comes from the bad event and it can add at most $O(q^2 )\cdot O(e^{-\eps nd}) \leq O(1)$, hence we have $\nu_1 = 1/\eps$. 
Finally, we prove the approximately scale invariant property.
Suppose the input satisfies $|x_i - x_i'| \leq a$ and $a\in (1/\sqrt{d}, 1)$, then we know the $L_1$-sensitivity satisfies $|\mathsf{fp}(x_i, p) - \mathsf{fp}(x_i', p)| \leq \lceil ap\rceil + 2$. Since we add a discrete Laplace variable of order $\eps/p$, the protocol is at lest $(2a\eps, 1/\poly(n,d))$ private.
\end{proof}

==> main_text/conclusion.tex <==
\section{Conclusion, Societal Impact, and Limitations}
\label{sec:conclusion}
This work provides a shuffle private protocol for summing vectors with bounded $\ell_2$ sensitivity and applies it to construct shuffle private stochastic convex optimization algorithms. As this is theoretical work on a general problem, it is difficult to draw a direct line between it and concrete societal concerns. However, a general criticism of private machine learning is that, by broadening the scope and quantity of data available for learning, it may contribute to increased surveillance; in that regard, this paper is no exception. Turning to more technical limitations, one drawback of our work is that it relies on the existence of a trusted shuffler, though we note that this assumption is made by all work on shuffle privacy. In addition, we have not optimized our algorithms for communication complexity. Adapting more communication-efficient summation protocols~\cite{BBGN19, GKMP20} to satisfy the instance-specific guarantee of Lemma~\ref{lem:ssum} may be a path to reducing the communication complexity in future work.

==> main_text/reduction.tex <==

\iffalse
\begin{definition}
\label{def:sum-property}
We say a \textsc{Single-Sum} protocol $\hat{\mathcal{P}}$ is $\nu_1$-biased, if for every function $f: \mathcal{X}\rightarrow [-1,1]$ and every input data $x_1, \cdots, x_n \in \mathcal{X}$, one has
\[
\left|\E{}{\hat{\mathcal{P}}(f, X)} - \sum_{i=1}^{n}f(x_i)\right| \leq \nu_1
\]
%\jm{Switch $\alpha$ to $\nu_1$? Maybe also good to make it clear that $\mathcal{P}$ depends on $f$, i.e. $\hat{\mathcal{P}}(f, X)$. In this definition, it is stated as the $\nu_1$-biased is defined for each $f,X$ pair. Is this intended or you want to define it for all $f, X$? The quantifiers are missing for later definitions.}
The \textsc{Single-Sum} protocol is $\nu_2$-bounded, if
\[
\E{}{\left\|\hat{\mathcal{P}}(f, X) -\sum_{i=1}^{n}f(x_i)\right\|_2^2} \leq \nu_2
\]
Moreover, we say the protocol is $\nu_3$-approximately scale invariant, if for any $\alpha \in (1/\sqrt{d}, 2]$, when the $L_1$-sensitivity of input dataset satisfies $|f(x_i) - f(x_i')| < \alpha$ for any $i \in [n]$, then the \textsc{Single-Sum} protocol is $(\nu_3\alpha\eps, \delta)$-differentially private %\jm{We need to be consistent with the privacy notion, maybe always use $(,)$-DP or $(,)$-differentially private}.
\end{definition}


We next show all previous protocols are (at most) $1/\poly(n,d)$-biased, $O(\frac{1}{\eps}\log \frac{n}{\delta})$-bounded and $O(1)$-approximately scale invariant, The proof is deferred to Appendix~\ref{sec:app-protocol}.
\begin{lemma}
\label{lem:sum-property}
We have
\begin{itemize}
    \item The CSU protocol \cite{CSU+19} is $\nu_1$-biased, $\nu_2$-bounded \jm{Stay consistent with dashes: $\nu_2$-bounded} and $\nu_3$-approximately scale invariant with $\nu_1 = 0$, $\nu_2 = \frac{1}{\eps}\log \frac{n}{\delta}$, $\nu_3 = O(1)$.
    \item The BBGN protocol \cite{BBGN19} is $\nu_1$-biased, $\nu_2$-bounded and $\nu_3$-approximately scale invariant with $\nu_1 = 1/\poly(n, d)$, $\nu_2 = \frac{1}{\eps}$ and $\nu_3 = O(1)$.
    \item The KLS protocol \cite{KLS21} is $\nu_1$-biased, $\nu_2$-bounded and $\nu_3$-approximately scale invariant with $\nu_1 = 1/\poly(n, d)$, $\nu_2 = \frac{1}{\eps}$ and $\nu_3 = O(1)$.\Binghui{To check.}
\end{itemize}
\end{lemma}



\begin{theorem}
\label{thm:shuffle-sum}
For every $ n > 0$, $\eps > 0$, $\delta \gtrsim n^{-O(\log n)}$, suppose the \textsc{Single-Sum} protocol is $\nu_1$-biased, $\nu_2$-bounded and $\nu_3$-approximately scale invariant with $\nu_1 = 1/\poly(n,d)$, $\nu_2 = O\left(\frac{1}{\eps}\log \frac{n}{\delta}\right)$ and $\nu_3 = O(1)$.
Then for every $X = (x_1,\cdots, x_n) \in \mathcal{X}^n$, every function $f: \mathcal{X} \rightarrow \mathbb{R}^{d}$ with $\|f(x)\|_2\leq 1$, the output $\mathcal{P}(X)$ of the shuffle protocol $P$ in Algorithm~\ref{alg:shuffle_sum} satisfies
\begin{align}
\label{eq:vector-sum1}
\left\|\E{}{P(X)} - \sum_{i=1}^{n}f(x_i) \right\|_2 \leq \sqrt{d} \nu_1 \lesssim \frac{1}{\poly(n, d)}
\end{align}
and
\begin{align}
\label{eq:vector-sum2}
\E{}{\left\|P(X) -\sum_{i=1}^{n}f(x_i)\right\|_2^2} \leq d\nu_2 =  O\left(\frac{d}{\eps^2}\log^2 \frac{n}{\delta}\right).
\end{align}
Moreover, the protocol is $(O(\eps\log(1/\delta)), O(d\delta))$-differentially private. 
\end{theorem}

\fi



%The CSU protocol \cite{CSU+19} has the following property.
%\begin{lemma}[Adapt from Theorem 2.1 of ~\cite{CSU+19}]
%\label{lem:csu-accuracy}
%For every $\eps \in (0, 1)$, and every $\delta \gtrsim 2^{\eps n}$ and every function $f: \mathcal{X}\rightarrow [0,1]$, there is a protocol $\mathcal{P}$ in the shuffle model that is $(\eps, \delta)$-differentially private and for every $X = (x_1, \cdots, x_n)\in \mathcal{X}^{n}$, we have
%\[
%\E{}{\mathcal{P}(X)} = \sum_{i=1}^{n}f(x_i)
%\]
%and 
%\[
%\E{}{\left| \mathcal{P}(X) - \sum_{i=1}^{n}f(x_i) \right|^2} = O\left(\frac{1}{\eps^2}\log^2 \frac{n}{\delta}\right)
%\]
%\Binghui{Albert, please check the following part.}
%Furthermore, for $\alpha \in (1/d, 1)$, if the function $f$ satisfies $|f(x_i) - f(x_i')| < \alpha$ holds for any $i \in [n]$ and $x_i' \in \mathcal{X}$, then the CSU protocol is $(\alpha \eps, \delta)$-differential private. \Albert{Is this all you need? It seems like you could use this proof structure to argue that variance of Laplace mechanism just needs to be scaled to L2 sensitivity. But is that true?}
%\end{lemma}
%\fi
%\begin{proof}
%\Binghui{The second equation and the second part requires a formal proof.}
%\end{proof}






%The key to our proof is the following version of composition theorem, we provide the proof in Appendix~\ref{sec:app-advance}.
\Albert{How about rephrasing the result like this: ``Let $X_1,\dots,X_d, Y_1,\dots,Y_d$ be (independent?) random variables. If there are finite $\eps_j,\delta_j$ such that $D^{\delta_j}_\infty (X_j||Y_j)<\eps_j$, then $D^{\delta}_\infty (\vec{X}||\vec{Y})<\eps$ for so-and-so $\eps,\delta$.'' I think this is what we need, since we have divergence bounds and not better privacy parameters per execution.}

\begin{theorem}[Generalization of Advanced Composition]
\label{thm:advance-composition}
Let $d \in \mathbb{Z}^{+}$ and $i \in [d]$, suppose algorithm $\mathcal{A}_{i}: \mathcal{X}^{n}\rightarrow \mathbb{R}$ satisfies
\[
\Pr[\mathcal{A}_i(S) \in M_i]\leq e^{\eps_i}\Pr[\mathcal{A}_i(S')] + \delta_i
\]
for any possible outcome set $M_i \subseteq \mathbb{R}$ and any neighbor datasets $S, S' \subseteq \mathcal{X}^{n}$.
%any dataset $S \subseteq \mathcal{X}^{n}$ 
%$(\eps_i, \delta_i)$-differentially private. 
Let  %$\eps_{\max} = \max\{\eps_1, \cdots, \eps_k\}$, 
\[
\eps' =  \sum_{i=1}^{d} \eps_i(e^{\eps_i} - 1) + 2\sqrt{\log(1/\gamma)\sum_{i=1}^{d}\eps_i^{2}} %+ \eps_{\max}\log (1/\gamma),
\quad \text{and} \quad
\delta' = \sum_{i=1}^{d}\delta_i + \gamma.
\]
Then the composition $(\mathcal{A}_1(S), \cdots, \mathcal{A}_{k}(S))$ satisfies
\begin{align*}
    \Pr[(\mathcal{A}_1(S), \cdots, \mathcal{A}_d(S)\in M]\leq e^{\eps'}\Pr[(\mathcal{A}_1(S), \cdots, \mathcal{A}_d(S)\in M] + \delta'
\end{align*}
for any possible outcome set $M \subseteq \mathbb{R}^{k}$.
%is $(\eps', \delta')$-differentially private and
%For all $\eps, \delta', \delta \geq 0$, the class of $(\eps, \delta)$ differential private mechanism satisfies $(\eps', \delta')$ differential privacy under $k$-fold adaptive composition, where
%where $\eps_{\max} = \max\{\eps_1, \cdots, \eps_k\}$.
%\Binghui{Check later}
\end{theorem}

\begin{corollary}
\label{cor:advance-composition}
For any $i \in [d]$, suppose the algorithm $\mathcal{A}_{i}: \mathcal{X}^{n}\rightarrow \mathbb{R}$ satisfies 
\[
\Pr[\mathcal{A}_i(S) \in M_i]\leq e^{\eps_i}\Pr[\mathcal{A}_i(S')] + \delta_i
\]
for any neighbor datasets $S$, $S'$ and outcome set $M'\in\mathbb{R}$. Suppose $\sum_{i=1}^{d}\eps_i^2 \leq \eps^2 \leq O(1)$, then the composition $(\mathcal{A}_1(S), \cdots, \mathcal{A}_{d}(S))$ satisfies
\[
    \Pr[(\mathcal{A}_1(S), \cdots, \mathcal{A}_d(S)\in M]\leq e^{\eps'}\Pr[(\mathcal{A}_1(S), \cdots, \mathcal{A}_d(S)\in M] + \delta'
\]
with $\eps'=O(\eps\sqrt{\log(1/\delta)}),\delta'= (d+1)\delta$.
\end{corollary}

\begin{proof}[Proof of Claim~\ref{clm:privacy-reduction}]
\iffalse
For the accuracy guarantee, since we run a $\nu_1$-biased \textsc{Single-Sum} protocol for each coordinate $j \in [d]$, we have
\[
\left|\E{}{P(X)_j} - \sum_{i=1}^{n}f(x_i)_j\right| \leq \nu_1,
\]
and therefore %\jm{Are we proving an $\ell_1$ bound or $\ell_2$ bound here?}\Binghui{$\ell_2$ bound, add the norm now.}
\[
\left\|\E{}{P(X)} - \sum_{i=1}^{n}f(x_i)\right\|_2 \leq \sqrt{\sum_{j =1}^{d}\left(\E{}{P(X)_j} - \sum_{i=1}^{n}f(x_i)_j\right)^2} \leq \sqrt{d}\nu_1 \leq 1/\poly(n, d).
\]
Similarly, since the \textsc{Single-Sum} protocol is $\nu_2$-bounded, one has
\[
\E{}{\left\|P(X) -\sum_{i=1}^{n}f(x_i)\right\|^2} = \sum_{j =1}^{d}\E{}{\left|P(X)_j -\sum_{i=1}^{n}f(x_i)_j\right|^2}\leq d\nu_2 \leq O\left(\frac{d}{\eps^2}\log^2 \frac{n}{\delta}\right).
%\footnote{\Binghui{Note this does not directly follow the theorem statement of CSU~\cite{CSU+19}, we need a proof here}.}
\]
\fi

Fix any neighboring datasets $\vec{x}, \vec{x}'$. We assume without loss of generality that the datasets differ in the last coordinate, i.e., $ \vec{x}= (x_1, \cdots, x_{n-1}, x_n)$ and $\vec{x}' = (x_1, \cdots, x_{n-1}, x_n')$. %\jm{say we can wlog consider neighboring datasets differ in the last coordinate.} One has
\[
\left\|\sum_{i=1}^{n}x_i - \sum_{i=1}^{n}x_i'\right\|_2 = \left\|x_n - x_n'\right\|_2 \leq \sqrt{2}.
\]
\Matthew{The statement of Claim 3.3 says that $\vec{x}$ and $\vec{x'}$ are databases of scalars, but this analysis says they're vectors?}For each coordinate $j \in [d]$, we use $a_j$ to denote the difference in $j$-th coordinate, i.e.,
\[
a_j := \left(\sum_{i=1}^{n}x_{i, j} - \sum_{i=1}^{n}x_{i, j}'\right) = x_{i, j} - x_{i, j}'
\]
we then have 
$\sum_{i=1}^{n}a_j^2 \leq 2$. %\jm{$\sum$ typo}


For the central aggregator, 
%we partition all messages it receive into $d$ separate parts , where the $j$-th part contains all messages involving the $j$-th coordinate. 
%let $\Pi(\vec{x})$ (resp. $\Pi(\vec{x}')$) denote all messages it receives on dataset $\vec{x}$ (resp. $\vec{x}'$).
we write $\Pi(\vec{x}) = (\Pi(\vec{x})_1, \cdots, \Pi(\vec{x})_d)$, where $\Pi(\vec{x})_j$ contains all messages involving the $j$-th coordinate.
%We use $A_{X}$ (resp. $A_{X'}$) to denote the message received on dataset $X$ (resp. $X'$), and let $A_{X} = (A_{X, 1}, \cdots, A_{X,d})$, $A_{X'} = (A_{X', 1}, \cdots, A_{X',d})$. 
For each $j\in [d]$, we know that the input on $j$-th coordinate, $(x_{1,j}, \cdots, x_{n,j})$ and $(x_{1,j}', \cdots, x_{n,j}')$, differ in at most one entry across the two datasets, and $|x{n,j}' - x_{n, k}| = a_j$. 
Let 
$\eps_j = \max\{a_j\eps, \frac{1}{\sqrt{d}}\eps\}$,
%and
%\[
%B_j = \{M_j: \Pr[\Pi(\vec{x})_j = M_j] \geq e^{\eps_j}\Pr[\Pi(\vec{x}')_j = M_j\},
%\] 
%by the $\nu_3$-approximately scaling invariant property of the \textsc{Single-Sum} protocol, 
then we know that
\[
\Pr[\Pi(\vec{x})_j \in M_j] \leq e^{\eps_j}\Pr[\Pi(\vec{x}')_j \in M_j] + \delta
\]
holds for any $M_j$.
%one has $\Pr[\Pi(\vec{x})_j \in B_j] \leq \frac{1}{e^{\eps_j} - 1}\delta$. 

Furthermore, notice that
\[
\sum_{j \in [d]}\eps_j^2 = \sum_{j\in [d]}\max\left\{a_j\eps, \frac{1}{\sqrt{d}}\eps\right\}^2\leq \sum_{j \in [d]}a_j^2\eps^2 +  \frac{1}{d}\eps^2 \leq 2\eps^2 + \eps^2 = O(\eps^2)
\]
where the second step follows from $\max\{a, b\}^2 \leq a^2 + b^2, \forall a, b\in \mathbb{R}$, the third step follows $\sum_{j \in [d]}a_j^2 \leq 2$
%and the last step follows from $\nu_3 = O(1)$.
Let 
\[
\eps' = O(\eps\sqrt{\log(1/\delta)}), \quad \delta' = (d+1) \delta,
\]
%\[
%B = \left\{M = (M_1, \cdots, M_d): \Pr[A_X = M] \geq e^{\eps'}\Pr[A_{X'} = M] \text{ or } \Pr[A_X = M] \leq %e^{-\eps'}\Pr[A_{X'} = M]\right\},
%\] 
by the generalized advanced composition Theorem and Corollary~\ref{cor:advance-composition}, one has
\begin{align}
    \Pr[(\Pi(\vec{x})_1, \cdots, \Pi(\vec{x})_d) \in M] \leq e^{\eps'}\Pr[(\Pi(\vec{x}')_1, \cdots, \Pi(\vec{x}')_d) \in M] + \delta'.
    \label{eq:vector-sum3}
\end{align}
Since Eq.~\eqref{eq:vector-sum3} holds uniformly for all neighboring dataset $\vec{x}$ and $\vec{x}'$, we conclude that our protocol is $(\eps', \delta')$ differentially private.

%We are going to prove that for any $(M_1, \cdots, M_d)$, we 

%its input contains message from all $d$ coordinates, we provide privacy guarantee for each coordinate and use composition theorem. For any coordinate $j$, since the input data only differs by $a_j$, this part of message is $(a_j\eps, \delta)$-differential private by Lemma~\ref{lem:csu-accuracy}.
%\Binghui{Albert, please check this part. I guess it should be correct, but it seems we need to go into the rounding details}. 
%Using composition theorem (see Theorem~\ref{thm:advance-composition} and Corollary~\ref{cor:advance-composition}), we conclude the protocol is $(\eps \log(1/\delta), d\delta)$-differential private.

\end{proof}

%The algorithm for interactive shuffle model is shown in Algorithm~\ref{alg:isp_sgd} and the algorithm for sequential shuffle model is shown in Algorithm~\ref{alg:ssp_sgd}. 
